Phenomenological aspects of supergravity theories in de Sitter vacua

We introduce an $N=1$ supergravity model based on the gauged shift symmetry of a single chiral multiplet, which can be identified with the string dilaton or a compactification modulus. The model allows for a tunably small and positive value of the cosmological constant. The gravitino mass parameter and the dilaton Vacuum Expectation Value are separately tunable. In a second part we analyze the quantum consistency of these models. Recent work on anomalies in supergravity theories with Fayet-Iliopoulos terms was extended, such that their results can be interpreted from a field-theoretic point of view. We show that for certain values of the parameters the anomaly cancellation conditions are inconsistent with a TeV gravitino mass. In the third part the above model is used as a hidden sector for supersymmetry breaking. In its minimal version, the model leads to tachyonic scalar soft masses. This problem can however be circumvented by the introduction of an extra Pol\'onyi-like hidden sector field, or by allowing for non-canonical kinetic terms for the Standard Model fields, while maintaining the desirable features of the model. The resulting low energy spectrum consists of very light neutralinos, charginos and gluinos, while the squarks remain heavy, with the exception of the stop squark which can be as light as 2 TeV. Finally, we discus possibility that the shift symmetry is identified with known global symmetries of the MSSM. The particular cases where this global symmetry is Baryon minus Lepton number ($B-L$), or $3B-L$, which contain the known R-parity or matter parity of the MSSM, are analyzed in great detail. It is shown that the phenomenology is similar to the above case where the MSSM fields are inert, with the exception of the stop squark, which can be as light as $1.5$ TeV.

==> chapters/abstract/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: abstract.pdf
abstract.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: bare abstract_bare.pdf
bare: abstract_bare.pdf
abstract_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/abstract/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/abstract/abstract.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard abstract*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) abstract.pdf abstract_bare.pdf

s:
	@echo gvim abstract.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/abstract/abstract.tex <==
\chapter{Abstract}                                 \label{ch:abstract}


Supersymmetry is the most promising theory that extends the Standard Model. 
Theories with local supersymmetry (supergravity) appear as the low energy effective physics of string theory.
Recently there has been great interest in finding de Sitter vacua of supergravity and string theory.
In this thesis, we present a new class of de Sitter vacua
in $\mathcal N=1$ supergravity, 
and we focus on the phenomenological implications of these models.

In the first part of the thesis we introduce supersymmetry and supergravity. 
Particular emphasis is put on spontaneous supersymmetry breaking 
and the Minimally Supersymmetric Standard Model (MSSM).
We introduce a model based on the gauged shift symmetry of a single chiral multiplet, 
which can be identified with the string dilaton or a compactification modulus.
The model allows for a tunably small and positive value of the cosmological constant.
The gravitino mass parameter and the dilaton Vacuum Expectation Value are seperately tunable.

For certain values of the parameters 
the vacuum is metastable, 
and it is shown that the tunneling rate to the false vacuum exceeds the lifetime of the universe.
Moreover, the scalar potential corresponds with one derived from D-branes in non-critical strings.
Finally, a dual version of this model is presented in terms of a linear multiplet containing a 2-index antisymmetric tensor.

In a second part we analyze the quantum consistency of these models. 
Recent work by Elvang, Freedman and K\"ors on anomalies in supergravity theories with Fayet-Iliopoulos terms
 was extended, such that their results can be interpreted from a field-theoretic point of view. 
Next, we show that for certain values of the parameters the anomaly cancellation conditions are inconsistent with a TeV gravitino mass.
 We elaborate on the relations between the Green-Schwarz counterterms and the gaugino mass parameters, 
and show how (by an appropriate K\"ahler transformation) the resulting contribution to the gaugino mass can be identified with one-loop gaugino mass parameters 
that are generated by anomaly mediation.

In the third part the above model (in the parameter range which is consistent with the anomaly cancellation conditions) 
is used as a hidden sector where spontaneous supersymmetry breaking occurs. 
This supersymmetry breaking is then communicated to the visible sector (MSSM) by gravity effects, and the resulting soft supersymmetry breaking terms are calculated.
In its minimal version, the model leads to tachyonic scalar soft masses. 
This problem can however be circumvented by the introduction of an extra Pol\'onyi-like hidden sector field, 
or by allowing for non-canonical kinetic terms for the Standard Model fields, while maintaining the desirable features of the model.
The resulting low energy spectrum consists of very light neutralinos, charginos and gluinos, 
while the squarks remain heavy, with the exception of the stop squark which can be as light as 2 TeV.

Finally, we discus possibility that the shift symmetry is identified with known
global symmetries of the MSSM. The particular cases where this global symmetry is Baryon minus Lepton number ($B-L$), or $3B-L$, 
which contain the known R-parity or matter parity of the MSSM, are analyzed in great detail.
The latter combination has also the advantage of forbidding all dimension-four
and dimension-five operators violating baryon or lepton number in the MSSM. 
It is shown that the phenomenology is similar to the above case where the MSSM fields are inert, with the exception of the stop squark, which can be as light as $1.5$ TeV.
Finally, it is shown that the problem of tachyonic scalar masses can not
be solved by the presence of the (positive) D-term contributions to the scalar
potential, proportional to the charge of the MSSM superfields under the shift
symmetry.



\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/chargedMSSM/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: chargedMSSM.pdf
chargedMSSM.pdf: 
	( cd "$(MAINDIR)" && make chapters/chargedMSSM/$@ )

.PHONY: bare chargedMSSM_bare.pdf
bare: chargedMSSM_bare.pdf
chargedMSSM_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/chargedMSSM/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/chargedMSSM/chargedMSSM.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard chargedMSSM*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) chargedMSSM.pdf chargedMSSM_bare.pdf

s:
	@echo gvim chargedMSSM.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/commentsonp1/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: commentsonp1.pdf
commentsonp1.pdf: 
	( cd "$(MAINDIR)" && make chapters/commentsonp1/$@ )

.PHONY: bare commentsonp1_bare.pdf
bare: commentsonp1_bare.pdf
commentsonp1_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/commentsonp1/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/commentsonp1/commentsonp1.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard commentsonp1*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) commentsonp1.pdf commentsonp1_bare.pdf

s:
	@echo gvim commentsonp1.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/conclusion/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: conclusion.pdf
conclusion.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: bare conclusion_bare.pdf
bare: conclusion_bare.pdf
conclusion_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/conclusion/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/conclusion/conclusion.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard conclusion*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) conclusion.pdf conclusion_bare.pdf

s:
	@echo gvim conclusion.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/curriculum/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:12 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: curriculum.pdf
curriculum.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: bare curriculum_bare.pdf
bare: curriculum_bare.pdf
curriculum_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/curriculum/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/curriculum/curriculum.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard curriculum*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) curriculum.pdf curriculum_bare.pdf

s:
	@echo gvim curriculum.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/curriculum/curriculum.tex <==
\chapter{This is curriculum}\label{ch:curriculum}

\ldots

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/dS/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: dS.pdf
dS.pdf: 
	( cd "$(MAINDIR)" && make chapters/dS/$@ )

.PHONY: bare dS_bare.pdf
bare: dS_bare.pdf
dS_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/dS/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/dS/dS.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard dS*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) dS.pdf dS_bare.pdf

s:
	@echo gvim dS.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/introduction/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:12 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: introduction.pdf
introduction.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: bare introduction_bare.pdf
bare: introduction_bare.pdf
introduction_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/introduction/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/introduction/introduction.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard introduction*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) introduction.pdf introduction_bare.pdf

s:
	@echo gvim introduction.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: manual.pdf
manual.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: bare manual_bare.pdf
bare: manual_bare.pdf
manual_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/manual/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/manual/manual.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard manual*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) manual.pdf manual_bare.pdf

s:
	@echo gvim manual.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/manual/manual.tex <==
\chapter{Manual}\label{ch:manual}


\ldots

\section{Tips and Tricks}


\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\\makefrontcovergeneral} and \texttt{\\makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\\defaultlbleed} and \texttt{\\defaultrbleed} respectively.


\subsection{Finetuning the backref package}

Finetuning the backref package (when \textbf{not} using biblatex). Add the
following to your preamble:

\begin{verbatim}
% See [http://n2.nabble.com/backref-td478438.html]:
% simple backref command redefinition to avoid double entries
\makeatletter
\ifadsphd@biblatex\else
  \ifadsphd@pagebackref%
    \renewcommand*{\backref}[1]{}
    % redefinition of the actually used \backrefalt 
    \renewcommand*{\backrefalt}[4]{% 
    \ifcase #1 % 
       % case: not cited 
    \or 
       % case: cited on exactly one page 
       Cited on page~#2.
    \else 
       % case: cited on multiple pages 
       Cited on pages~#2.
    \fi}
  \else
    \renewcommand*{\backref}[1]{}
    % redefinition of the actually used \backrefalt 
    \renewcommand*{\backrefalt}[4]{% 
    \ifcase #1 % 
       % case: not cited 
    \or 
       % case: cited on exactly one page 
       Cited in Section~#2.
    \else 
       % case: cited on multiple pages 
       Cited in Sections~#2.
    \fi}
  \fi
\fi
\makeatother
\end{verbatim}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/notation/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: notation.pdf
notation.pdf: 
	( cd "$(MAINDIR)" && make chapters/notation/$@ )

.PHONY: bare notation_bare.pdf
bare: notation_bare.pdf
notation_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/notation/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/notation/notation.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard notation*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) notation.pdf notation_bare.pdf

s:
	@echo gvim notation.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/notation/notation.tex <==
\chapter{Notation}
\todo{To Toine: Deze appendix moet ik eens opnieuw bekijken. Ik weet eerlijkgezegd niet zo goed wat hierin moet komen aangezien ik in deze thesis de notatie van uw boek probeer aan te houden.}

\section{The supersymmetric Lagrangian} \label{Appendix:SUSYLagrangian}
The Lagrangian is then given by
\begin{align} \mathcal L &= \mathcal L_{\text{kin,chir}} + \mathcal L_{\text{kin,gauge}} + \mathcal L_{\text{pot,chir}}.\end{align}
where the kinetic terms for the chiral multiplets are given by
\begin{align} \mathcal L_{\text{kin,chir}} =& g_{\alpha \bar \beta} \left[ -D_\mu Z^\alpha D^\mu \bar Z^{\bar \beta} - \frac{1}{2}\bar \chi^\alpha P_L \cancel{\nabla} \chi^{\bar \beta} - \frac{1}{2} \bar \chi^{\bar \beta} P_R \cancel \nabla \chi^\alpha \right. \notag \\
& \ \ \left. +  \left(F^\alpha - \frac{1}{2} \Gamma^{\alpha}_{\gamma \beta} \bar \chi^\gamma P_L \chi^\beta \right) \left( \bar F^{\bar \beta} - \frac{1}{2} \Gamma^{\bar \beta}_{\bar \gamma \bar \alpha} \bar \chi^{\bar \gamma} P_R \chi^{\bar \alpha} \right) \right] \notag \\
& \ \ + \frac{1}{4} R_{\alpha \beta \bar \gamma \bar \delta} \bar \chi^\alpha P_L \chi^\beta \bar \chi^{\bar \gamma} P_R \chi^{\bar \delta} \notag \\
& \ \ - D^A \mathcal P_A - \sqrt{2} \bar \lambda^A \left( P_L \chi^\alpha k_{A \alpha} + P_R \chi^{\bar \beta} k_{A \bar \beta} \right).
\end{align} 
The kinetic (and potential) terms for the gauge multiplets are given by
\begin{align}
\mathcal L_{\text{kin,gauge}} = & - \frac{1}{4} \re f_{AB} \left(  2 \bar \lambda^A \cancel D \lambda^B + F_{\mu \nu}^A F^{\mu \nu \ B} - 2D^A D^B\right) \notag \\
& \ \ + \frac{1}{8} \im f_{AB} \epsilon^{\mu \nu \rho \sigma} F_{\mu \nu}^A F_{\rho \sigma}^B + \frac{1}{4} i \left( \im D_\mu f_{AB} \bar \lambda^A \gamma_* \gamma^\mu \lambda^B \right) \notag \\
& \ \ + \frac{1}{2 \sqrt 2} f_{AB\alpha} \bar \chi^\alpha \left( - \frac{1}{2} \gamma^{\mu \nu} F_{\mu \nu}^{- \ A} + i D^A \right) P_L \lambda^B - \frac{1}{4} f_{AB\alpha} F^\alpha \bar \lambda^A P_L \lambda^B \notag \\
& \ \ + \frac{1}{8} f_{AB\alpha\beta} \bar \chi^\alpha  P_L \chi^\beta \bar \lambda^A P_ \lambda^B + \text{h.c.}
\end{align}
The potential terms for the chiral multiplets are given by
\begin{align}
 \mathcal L_{\text{pot,chir}} = W_\alpha F^\alpha - \frac{1}{2} W_{\alpha \beta} \bar \chi^\alpha P_L \chi^\beta + \text{h.c.}
\end{align}
Here, the chiral multiplets are labelled by a Greek index $\alpha, \beta, \dots$ and the gauge multiplets carry a capital Roman index $A,B,\dots$ . $P_L$ ($P_R$) is the left-handed (right-handed) projection operator. 
$\gamma_*$ is given by
\begin{align}
 \gamma_* = i \gamma_0 \gamma_1 \gamma_2 \gamma_3, \label{gammastar}
\end{align}
where $\gamma_\mu$ are the gamma matrices.
The metric is given by
\begin{align}
 g_{\alpha \bar \beta} = \partial_\alpha \partial_{\bar \beta} K(Z, \bar Z),
\end{align}
The connection components are given by
\begin{align}
 \Gamma^\alpha_{\beta \gamma} &= g^{\alpha \bar \delta} \partial_\beta g_{\gamma \bar \delta}, \notag\\
 \Gamma^{\bar \alpha}_{ \bar \beta \bar \gamma} &= g^{\delta \bar \alpha} \partial_{\bar \beta} g_{ \delta \bar \gamma}. \label{connection components}
\end{align}
All other connection components vanish (i.e. $\Gamma^\alpha_{\beta \bar \gamma} = \Gamma^{\bar \alpha}_{\bar \beta \gamma} = 0$). $R_{\alpha \bar \beta \gamma \bar \delta} $ is the curvature tensor.

The covariant derivatives are given by
\begin{align}
 D_\mu Z^\alpha &= \partial_\mu Z^\alpha - A_\mu^A k_A^\alpha, \notag \\
 P_L \nabla_\mu \chi^\alpha&= \partial_\mu P_L \chi^\alpha - A_\mu^A \frac{\partial k_A^{\ \alpha}(Z) }{\partial Z^\beta} P_L \chi^\beta + \Gamma^\alpha_{\beta \gamma} P_L \chi^\gamma D_\mu Z^\beta, \notag \\
D_\mu \lambda^A &=\partial_\mu \lambda^A + A_\mu^{\ \beta} f_{BC}^{\ \ A} \lambda^C, \notag \\
%F_{\mu \nu}^A &= \partial_\mu A_\nu^A - \partial_\nu A_\mu^A + f_{BC}^{\ \ A} A_\mu^B A_\nu^C, \notag \\
D_\mu f_{AB} &= \partial_\mu f_{AB} - 2 A_\mu^C f_{C(A}^{\ \ D} f_{B)D}.
\end{align}

\todo{cite somewhere:  E.~Witten,``Dynamical Breaking of Supersymmetry,''  Nucl.\ Phys.\ B {\bf 188} (1981) 513;}
\todo{cite somewhere:  W.~Fischler, H.~P.~Nilles, J.~Polchinski, S.~Raby and L.~Susskind,``Vanishing Renormalization of the D Term in Supersymmetric U(1) Theories,''  Phys.\ Rev.\ Lett.\  {\bf 47} (1981) 757.  }

\cleardoublepage


==> chapters/preface/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: preface.pdf
preface.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: bare preface_bare.pdf
bare: preface_bare.pdf
preface_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/preface/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/preface/preface.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard preface*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) preface.pdf preface_bare.pdf

s:
	@echo gvim preface.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/preface/preface.tex <==
\chapter*{Dankwoord}                                  \label{ch:preface}

Een thesis schrijf je niet alleen, daarom ook een kort dankwoord.
Graag wil ik hier iedereen bedanken die op de \'e\'en of andere manier heeft bijgedragen aan deze scriptie.

Ten eerste zou ik graag mijn ouders bedanken, die me altijd gemotiveerd hebben om verder te studeren en om mijn dromen te volgen.
Zonder hen zou ik hier niet staan, letterlijk en figuurlijk.

Graag zou ik ook mijn promotors Antoine Van Proeyen en Ignatios Antoniadis bedanken.
Enerzijds is er Toine, wie voor mij een grote inspiratiebron is geweest in mijn keuze om een doctoraatsopleiding te volgen,
en wie altijd klaar stond om mij te begeleiden met zowel mijn administratieve als fysicavragen.
I'd also like to thank Ignatios who, despite having a very loaded travel schedule, always found a way to advice me on this thesis.\footnote{
In one occasion, we even met on the train from Geneva to Bern when Ignatios was traveling from Paris, on a holiday (Jeûne Genevois), just so we could discuss our project. 
The result of this train ride is section~\ref{sec:Anomalies-gauginomass}.}

Naast mijn promotors, zou ik ook graag de andere leden van mijn examencommissie bedanken, namelijk Nikolay Bobev, Mark Fannes, Thomas Hertog, Christian Maes, Thomas Van Riet en Jean-Pierre Derendinger,
voor het doornemen van mijn thesis, het bijwonen van mijn interne verdediging, en de bijhorende feedback op een eerste versie van deze thesis.

Next, I'd like to thank the mathematics department at Geneva University, with in particular Anton Alekseev, for their hospitality during the last two years of my thesis. 

Being at CERN, I have also had the opportunity to discuss with (or rather, learn from) Fabio, Jean-Pierre, John, Luis, and Sergio.
Besides the endless discussions about physics, I have also had the opportunity to meet the most amazing people in Geneva that educated me in the school of life.
In particular, many of the most amazing weekends of my life were spent with 
Bruno, Carolyn, Claire, Dani, Garoe, Jabu, Cadi, Iikka, Javi, Jose, Helina, Luis, MCRaf, Sabri, Tincho, Tito, Tom, and many more.
A special thanks goes to Kevin, Marco, Matthi, Pedro and Subodh for their support during the final stages of this thesis.

Finally, I'd like to thank my brother Gert, who is also pursuing a Ph.D. in Physics, for not finishing his thesis before mine, although it took me nearly five years.

This work was supported in part by the European Commission under the ERC Advanced Grant 226371.
This work was also partly supported by the NCCR SwissMAP, funded by the Swiss National Science Foundation.

%\instructionspreface
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/softterms/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:11 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: softterms.pdf
softterms.pdf: 
	( cd "$(MAINDIR)" && make chapters/softterms/$@ )

.PHONY: bare softterms_bare.pdf
bare: softterms_bare.pdf
softterms_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/softterms/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/softterms/softterms.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard softterms*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) softterms.pdf softterms_bare.pdf

s:
	@echo gvim softterms.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/supergravity/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:12 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: supergravity.pdf
supergravity.pdf: 
	( cd "$(MAINDIR)" && make chapters/supergravity/$@ )

.PHONY: bare supergravity_bare.pdf
bare: supergravity_bare.pdf
supergravity_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/supergravity/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/supergravity/supergravity.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard supergravity*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) supergravity.pdf supergravity_bare.pdf

s:
	@echo gvim supergravity.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> chapters/supersymmetry/Makefile <==
# Autogenerated Makefile, Mon Apr 18 16:55:12 CEST 2016.

MAINDIR = /home/rob/Thesis/adsphd-master

.PHONY: supersymmetry.pdf
supersymmetry.pdf: 
	( cd "$(MAINDIR)" && make chapters/supersymmetry/$@ )

.PHONY: bare supersymmetry_bare.pdf
bare: supersymmetry_bare.pdf
supersymmetry_bare.pdf: 
	( cd "$(MAINDIR)" && make chapters/supersymmetry/$@ )

.PHONY: image
image: 
	@if [ -f image/Makefile ]; then (cd image  && make); \
		else echo No Makefile found for /home/rob/Thesis/adsphd-master/image ...; fi;

.PHONY: figurelist
figurelist:
	@( cd $(MAINDIR) && make --no-print-directory $@ TEXFILE=chapters/supersymmetry/supersymmetry.tex )

.PHONY: clean
clean:
	$(RM) $(foreach ext, .toc .aux .log .bbl .blg .log .lof .lot .ilg .out .glo .gls .nlo .nls .brf .ist .glg .synctex.gz .tgz .idx .ind -blx.bib .fdb_latexmk .run.xml .bcf, $(wildcard supersymmetry*$(ext)))

.PHONY: realclean
realclean: clean
	$(RM) supersymmetry.pdf supersymmetry_bare.pdf

s:
	@echo gvim supersymmetry.tex allpapers.bib defs.tex  > $@
	@chmod +x $@
	@echo You can now start using ./s


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

